A Survey on Congestion Control and Scheduling for Multipath TCP: Machine Learning vs Classical Approaches

Multipath TCP (MPTCP) has been widely used as an efficient way for communication in many applications. Data centers, smartphones, and network operators use MPTCP to balance the traffic in a network efficiently. MPTCP is an extension of TCP (Transmission Control Protocol), which provides multiple paths, leading to higher throughput and low latency. Although MPTCP has shown better performance than TCP in many applications, it has its own challenges. The network can become congested due to heavy traffic in the multiple paths (subflows) if the subflow rates are not determined correctly. Moreover, communication latency can occur if the packets are not scheduled correctly between the subflows. This paper reviews techniques to solve the above-mentioned problems based on two main approaches; non data-driven (classical) and data-driven (Machine Learning) approaches. This paper compares these two approaches and highlights their strengths and weaknesses with a view to motivating future researchers in this exciting area of machine learning for communications. This paper also provides details on the simulation of MPTCP and its implementations in real environments.

==> paper_layout.tex <==

https://fedcsis.org/for_authors/instructions

Abstract -0.2
In progress Add remaining references to the preliminary sections 
In progress  add figures preliminary for example LSTM , Actor critics Deep CC , one figure from scheduler, one from traditional CC in MPTCP,
In progress equation to policy gradient, add equation and figure to RL,  etc

*Background or Terminology 0.5 to 1 page 
*slow start
*AIMD
*RL and DRL actor critic


*Traditional TCP vs Multipath TCP - 1 page, , 2-3 ref
*Major Drawbacks of Traditional TCP 
*Packet loss
*Packet Delay
*Out of order packets
*Highest Round Trip Time

*Overview of MPTCP - 1 page, 5 ref
  * What is MPTCP
  * Congestion Control
  * Scheduling
  * High Throughput
   *Low Latency


*Congestion Control of MPTCP - 4 pages, 20 ref  : 6/30
*Classical based approaches
*Machine Learning approaches
*add table fix issues 
*add preliminary section

*Scheduling of MPTCP - 2 pages, 5  ref:  july 2
*Classical approaches
*ML based approaches

*Controlling both Congestion and Scheduling of MPTCP -0.5, 3-5 ref
*Classical approaches
*ML based approaches

*Implementation of MPTCP:
*NS3
Real hardware (kernel)

FUture work - 1 page


Conclusion - o.3 page



